Learning from Successful and Failed Demonstrations via Optimization

Learning from Demonstration (LfD) is a popular approach that allows humans to teach robots new skills by showing the correct way(s) of performing the desired skill. Human-provided demonstrations, however, are not always optimal and the teacher usually addresses this issue by discarding or replacing sub-optimal (noisy or faulty) demonstrations. We propose a novel LfD representation that learns from both successful and failed demonstrations of a skill. Our approach encodes the two subsets of captured demonstrations (labeled by the teacher) into a statistical skill model, constructs a set of quadratic costs, and finds an optimal reproduction of the skill under novel problem conditions (i.e. constraints). The optimal reproduction balances convergence towards successful examples and divergence from failed examples. We evaluate our approach through several 2D and 3D experiments in real-world using a UR5e manipulator arm and also show that it can reproduce a skill from only failed demonstrations. The benefits of exploiting both failed and successful demonstrations are shown through comparison with two existing LfD approaches. We also compare our approach against an existing skill refinement method and show its capabilities in a multi-coordinate setting.

==> old_method.tex <==

\section{Basic Method}
Consider a simple reaching task. There are many possible methods for which this reaching task may be accomplished, as shown below.

 \begin{figure}[ht]
\centering
\includegraphics[trim=0 0em 0 0, clip, width=0.95\textwidth]{all_good.png}
\caption{\small{Basic reaching motion shown over five demonstrations.}} \label{demos}
\end{figure}

In the scene where these demonstration were recorded, all were considered successful demonstrations. However, consider a new scene with an obstacle placed at (0.5, 0). Now, two of these demonstrations would be considered failures. This would leave us with 3 demonstrations to learn from. If we were to use methods that use the mean of the given demonstrations, the mean would be placed near (0.5, 0) and possibly interact with an obstacle, leading to a failed reproduction. I propose that instead of discarding the failed demonstrations in this scene, we use them to learn how to move away from failure. If we were to create a model of the probability of success across time and space, we could use that model to create a reproduction with the maximum likelihood of success. This model would have many desirable features, like strong generalization and noise filtering. The reproduction would have three objectives: maximization of probability of success, minimization of the spring energy between points, and minimization of constrained initial, final, or via-points using strong attractors. This is modeled as the cost function:
\begin{equation}
    C(\vect{X}) = G(\vect{X}) + K(\vect{X}) - S(\vect{X})
\end{equation}
where $\vect{X}$ is the trajectory, $G$ measures the satisfaction of the trajectory according to its constraints, $K$ measures the spring energy between points of the trajectory, and $S$ is a measure of the likelihood of success of the trajectory. $G$ is modeled as
\begin{equation}
    G(\vect{X}) = 100 \sum_{a \in A} \exp{||x_i - a||}
\end{equation}
where $A$ is the set of constraints with indices $i$ and locations $a$. $K$ is modeled as
\begin{equation}
    K(\vect{X}) = \frac{k}{2} \sum_{i = 0}^{I - 1} ||x_i - x_{i + 1}||^2
\end{equation}
where $k$ is the spring constant and $I$ is the total number of indices. $S$ is modeled as
\begin{equation}
    S(\vect{X}) = \sum_{i = 0}^{I} \sum_{d \in D} (-1)^b \mathcal{N}(x_i; \mu_{di}, \sigma_d)
\end{equation}
where $D$ is the set of all demonstrations, $b$ is a Boolean which indicates whether the demonstration is a failed demonstration. The success is drawn from a Gaussian probability density function $\mathcal{N}$ whose mean and standard deviation are calculated as the demonstration's location and a constant which indicates the demonstration's spread. To find the highest success trajectory, the following optimization is performed:
\begin{equation*}
\begin{aligned}
& \underset{\vect{X}}{\text{minimize}}
& & C({\vect{X}}) \\
& \text{subject to}
& & A 
\end{aligned}
\end{equation*}

 \begin{figure}[ht]
\centering
\includegraphics[trim=0 0em 0 0, clip, width=0.45\textwidth]{mean_traj.png}
\includegraphics[trim=0 0em 0 0, clip, width=0.45\textwidth]{highest success traj k2=3.0.png}
\caption{\small{Basic reaching motion in a new scene where some demonstrations fail. Using the mean of successes is shown on the left, and may result in failure. Using LFFD is shown on the right, which is successful.}} \label{basic_repros}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[trim=0 0em 0 0, clip, width=0.95\textwidth]{prbs dim 0.png}
\caption{\small{Heatmap of success probability for reaching task with failed demonstrations.}} \label{basic_heatmap}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[trim=0 0em 0 0, clip, width=0.95\textwidth]{highest success traj k2=250.0.png}
\caption{\small{Figure showing generalization ability of LFFD.}} \label{general_repro}
\end{figure}

 \begin{figure}[ht]
\centering
\includegraphics[trim=0 0em 0 0, clip, width=0.3\textwidth]{highest success traj k2=2.5.png}
\includegraphics[trim=0 0em 0 0, clip, width=0.3\textwidth]{highest success traj k2=0.000152587890625.png}
\includegraphics[trim=0 0em 0 0, clip, width=0.3\textwidth]{highest success traj k2=4.76837158203125e-06.png}
\caption{\small{Examples showing noise filtering as well as effect of $k$ tuning, with overtuned (left), undertuned (right), and properly tuned (center) reproductions.}} \label{noise_repros}
\end{figure}
